It Ain't That Bad: Understanding the Mysterious Performance Drop in OOD Generalization for Generative Transformer Models

Large language models (LLMs) have achieved remarkable proficiency on solving diverse problems. However, their generalization ability is not always satisfying and the generalization problem is common for generative transformer models in general. Researchers take basic mathematical tasks like n-digit addition or multiplication as important perspectives for investigating their generalization behaviors. It is observed that when training models on n-digit operations (e.g., additions) in which both input operands are n-digit in length, models generalize successfully on unseen n-digit inputs (in-distribution (ID) generalization), but fail miserably on longer, unseen cases (out-of-distribution (OOD) generalization). We bring this unexplained performance drop into attention and ask whether there is systematic OOD generalization. Towards understanding LLMs, we train various smaller language models which may share the same underlying mechanism. We discover that the strong ID generalization stems from structured representations, while behind the unsatisfying OOD performance, the models still exhibit clear learned algebraic structures. Specifically, these models map unseen OOD inputs to outputs with learned equivalence relations in the ID domain, which we call the equivalence generalization. These findings deepen our knowledge regarding the generalizability of generative models including LLMs, and provide insights into potential avenues for improvement.

==> img_tex/representation_structure_2d.tex <==
\begin{figure*}[tb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img/fig_addition_representation_100}
\par\end{centering}
\caption{Representation structure of the first four principal components in the addition operation. Figure \ref{fig:addition_representation_pca_2D}(a) to Figure \ref{fig:addition_representation_pca_2D}(d) represent the first to the fourth principal components of model with 100\% test accuracy, respectively.} 
\label{fig:addition_representation_pca_2D}
\end{figure*}

==> img_tex/training_curve_multiplication.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img/fig_training_curves_multiplication}
\par\end{centering}
\caption{Training curve in multiplication operation.}
\label{fig:training_curves_multiplication}
\end{figure}
